Multi-Task Contrastive Learning for 8192-Token Bilingual Text Embeddings

We introduce a novel suite of state-of-the-art bilingual text embedding models that are designed to support English and another target language. These models are capable of processing lengthy text inputs with up to 8192 tokens, making them highly versatile for a range of natural language processing tasks such as text retrieval, clustering, and semantic textual similarity (STS) calculations. By focusing on bilingual models and introducing a unique multi-task learning objective, we have significantly improved the model performance on STS tasks, which outperforms the capabilities of existing multilingual models in both target language understanding and cross-lingual evaluation tasks. Moreover, our bilingual models are more efficient, requiring fewer parameters and less memory due to their smaller vocabulary needs. Furthermore, we have expanded the Massive Text Embedding Benchmark (MTEB) to include benchmarks for German and Spanish embedding models. This integration aims to stimulate further research and advancement in text embedding technologies for these languages.

==> tables/ablation-study-mlm/merged-de-en.tex <==
\begin{tabular}{lcccc}
\toprule
 & jina-bert-de-results & bibert-results & mBERT-results & XLM-Roberta-results \\
\midrule
mean & \bfseries 0.575 & 0.554 & 0.530 & 0.536 \\
STS22 (de-en) & \bfseries 0.575 & 0.554 & 0.530 & 0.536 \\
\bottomrule
\end{tabular}


==> tables/ablation-study-mlm/merged-de.tex <==
\begin{tabular}{lcccc}
\toprule
 & jina-bert-de-results & bibert-results & mBERT-results & XLM-Roberta-results \\
\midrule
mean & 0.571 & \bfseries 0.601 & 0.553 & 0.551 \\
GermanDPR (de) & 0.738 & \bfseries 0.772 & 0.760 & 0.719 \\
GermanSTSBenchmark (de) & 0.768 & \bfseries 0.788 & 0.716 & 0.751 \\
MIRACL (de) & 0.600 & \bfseries 0.615 & 0.593 & 0.570 \\
PawsX (de) & 0.598 & \bfseries 0.606 & 0.604 & 0.599 \\
STS22 (de) & 0.527 & \bfseries 0.574 & 0.476 & 0.498 \\
XMarket (de) & 0.193 & \bfseries 0.251 & 0.172 & 0.167 \\
\bottomrule
\end{tabular}


==> tables/ablation-study-mlm/merged-en-de.tex <==
\begin{tabular}{lcccc}
\toprule
 & jina-bert-de-results & bibert-results & mBERT-results & XLM-Roberta-results \\
\midrule
mean & 0.784 & \bfseries 0.793 & 0.704 & 0.731 \\
STS17 (en-de) & 0.784 & \bfseries 0.793 & 0.704 & 0.731 \\
\bottomrule
\end{tabular}


==> tables/ablation-study-mlm/merged-en.tex <==
\begin{tabular}{lcccc}
\toprule
 & jina-bert-de-results & bibert-results & mBERT-results & XLM-Roberta-results \\
\midrule
mean & 0.759 & \bfseries 0.764 & 0.748 & 0.751 \\
QuoraRetrieval (en) & 0.850 & \bfseries 0.863 & 0.832 & 0.846 \\
STS12 (en) & 0.703 & 0.714 & \bfseries 0.725 & 0.714 \\
STS13 (en) & 0.793 & \bfseries 0.834 & 0.793 & 0.811 \\
STS14 (en) & 0.736 & \bfseries 0.760 & 0.737 & 0.738 \\
STS15 (en) & 0.831 & \bfseries 0.842 & 0.832 & 0.839 \\
STS16 (en) & 0.796 & \bfseries 0.805 & 0.785 & 0.792 \\
STS17 (en) & \bfseries 0.860 & 0.857 & 0.842 & 0.833 \\
STS22 (en) & \bfseries 0.675 & 0.671 & 0.661 & 0.663 \\
TRECCOVID (en) & \bfseries 0.585 & 0.527 & 0.529 & 0.525 \\
\bottomrule
\end{tabular}


==> tables/english/all-trial.tex <==
\begin{tabular}{llcccc}
\toprule
 &  & de-pearson-6k & es-pearson-6k & jina-zh & multilingual-e5-base \\
\midrule
\multirow[c]{15}{*}{retrieval} & mean & 0.448 & 0.471 & 0.464 & \bfseries 0.493 \\
 & ArguAna (en) & 0.495 & \bfseries 0.501 & 0.395 & 0.442 \\
 & CQADupstackRetrieval (en) & 0.368 & \bfseries 0.388 & 0.365 & 0.385 \\
 & ClimateFEVER (en) & 0.222 & \bfseries 0.271 & 0.233 & 0.239 \\
 & DBPedia (en) & 0.320 & 0.326 & 0.302 & \bfseries 0.404 \\
 & FEVER (en) & 0.712 & 0.784 & 0.786 & \bfseries 0.794 \\
 & FiQA2018 (en) & 0.339 & 0.370 & 0.349 & \bfseries 0.382 \\
 & HotpotQA (en) & 0.548 & 0.595 & 0.603 & \bfseries 0.686 \\
 & NFCorpus (en) & 0.280 & 0.303 & 0.308 & \bfseries 0.325 \\
 & NQ (en) & 0.481 & 0.507 & 0.594 & \bfseries 0.600 \\
 & QuoraRetrieval (en) & 0.877 & 0.881 & \bfseries 0.885 & 0.876 \\
 & SCIDOCS (en) & 0.167 & 0.174 & \bfseries 0.179 & 0.172 \\
 & SciFact (en) & 0.609 & 0.627 & 0.612 & \bfseries 0.693 \\
 & TRECCOVID (en) & 0.648 & 0.674 & 0.638 & \bfseries 0.698 \\
 & Touche2020 (en) & 0.205 & 0.198 & \bfseries 0.242 & 0.214 \\
\multirow[c]{14}{*}{clustering} & mean & 0.403 & \bfseries 0.405 & 0.368 & 0.400 \\
 & ArxivClusteringP2P (en) & \bfseries 0.419 & 0.415 & 0.405 & 0.403 \\
 & ArxivClusteringS2S (en) & 0.325 & 0.322 & 0.315 & \bfseries 0.354 \\
 & BigPatentClustering (en) & 0.230 & 0.204 & 0.187 & \bfseries 0.240 \\
 & BiorxivClusteringP2P (en) & 0.344 & \bfseries 0.352 & 0.296 & 0.350 \\
 & BiorxivClusteringS2S (en) & 0.290 & 0.289 & 0.278 & \bfseries 0.295 \\
 & MedrxivClusteringP2P (en) & 0.316 & \bfseries 0.322 & 0.272 & 0.289 \\
 & MedrxivClusteringS2S (en) & \bfseries 0.294 & 0.288 & 0.263 & 0.284 \\
 & RedditClustering (en) & 0.479 & \bfseries 0.483 & 0.426 & 0.424 \\
 & RedditClusteringP2P (en) & 0.549 & \bfseries 0.560 & 0.530 & 0.552 \\
 & StackExchangeClustering (en) & \bfseries 0.555 & 0.554 & 0.532 & 0.553 \\
 & StackExchangeClusteringP2P (en) & 0.328 & \bfseries 0.336 & 0.325 & 0.305 \\
 & TwentyNewsgroupsClustering (en) & \bfseries 0.405 & 0.402 & 0.351 & 0.360 \\
 & WikiCitiesClustering (en) & 0.703 & 0.733 & 0.604 & \bfseries 0.796 \\
\multirow[c]{5}{*}{reranking} & mean & 0.549 & \bfseries 0.553 & 0.550 & 0.548 \\
 & AskUbuntuDupQuestions (en) & \bfseries 0.612 & \bfseries 0.612 & 0.610 & 0.582 \\
 & MindSmallReranking (en) & 0.303 & 0.306 & \bfseries 0.311 & 0.310 \\
 & SciDocsRR (en) & 0.786 & 0.793 & 0.786 & \bfseries 0.807 \\
 & StackOverflowDupQuestions (en) & 0.496 & \bfseries 0.502 & 0.492 & 0.494 \\
\multirow[c]{13}{*}{classification} & mean & 0.688 & 0.690 & 0.677 & \bfseries 0.730 \\
 & AmazonCounterfactualClassification (en) & 0.740 & 0.743 & 0.722 & \bfseries 0.790 \\
 & AmazonPolarityClassification (en) & 0.802 & 0.783 & 0.720 & \bfseries 0.906 \\
 & AmazonReviewsClassification (en) & 0.395 & 0.383 & 0.354 & \bfseries 0.445 \\
 & Banking77Classification (en) & 0.839 & \bfseries 0.853 & 0.842 & 0.827 \\
 & EmotionClassification (en) & 0.452 & 0.466 & \bfseries 0.473 & 0.452 \\
 & ImdbClassification (en) & 0.699 & 0.675 & 0.696 & \bfseries 0.855 \\
 & MTOPDomainClassification (en) & 0.903 & 0.904 & 0.894 & \bfseries 0.931 \\
 & MTOPIntentClassification (en) & 0.686 & 0.720 & 0.695 & \bfseries 0.753 \\
 & MassiveIntentClassification (en) & 0.696 & 0.708 & 0.696 & \bfseries 0.721 \\
 & MassiveScenarioClassification (en) & 0.741 & 0.738 & 0.740 & \bfseries 0.771 \\
 & ToxicConversationsClassification (en) & 0.695 & \bfseries 0.700 & 0.695 & 0.698 \\
 & TweetSentimentExtractionClassification (en) & \bfseries 0.613 & 0.611 & 0.594 & \bfseries 0.613 \\
\multirow[c]{4}{*}{pair-classification} & mean & 0.912 & \bfseries 0.914 & 0.906 & \bfseries 0.914 \\
 & SprintDuplicateQuestions (en) & \bfseries 0.998 & \bfseries 0.998 & \bfseries 0.998 & 0.997 \\
 & TwitterSemEval2015 (en) & 0.849 & 0.852 & 0.838 & \bfseries 0.856 \\
 & TwitterURLCorpus (en) & 0.890 & \bfseries 0.893 & 0.884 & 0.888 \\
\multirow[c]{11}{*}{sts} & mean & 0.820 & \bfseries 0.835 & 0.826 & 0.803 \\
 & BIOSSES (en) & 0.780 & 0.830 & 0.805 & \bfseries 0.851 \\
 & SICK-R (en) & 0.811 & 0.830 & \bfseries 0.862 & 0.785 \\
 & STS12 (en) & 0.801 & 0.816 & \bfseries 0.874 & 0.767 \\
 & STS13 (en) & 0.851 & \bfseries 0.868 & 0.818 & 0.780 \\
 & STS14 (en) & 0.811 & \bfseries 0.836 & 0.786 & 0.766 \\
 & STS15 (en) & 0.878 & \bfseries 0.887 & 0.861 & 0.882 \\
 & STS16 (en) & 0.836 & \bfseries 0.860 & 0.841 & 0.843 \\
 & STS17 (en) & \bfseries 0.893 & 0.886 & 0.886 & 0.878 \\
 & STS22 (en) & \bfseries 0.682 & 0.656 & 0.672 & 0.618 \\
 & STSBenchmark (en) & 0.862 & \bfseries 0.878 & 0.858 & 0.856 \\
\multirow[c]{2}{*}{summarization} & mean & \bfseries 0.318 & 0.299 & 0.313 & 0.301 \\
 & SummEval (en) & \bfseries 0.318 & 0.299 & 0.313 & 0.301 \\
\bottomrule
\end{tabular}


==> tables/english/classification.tex <==
\begin{tabular}{lcccc}
\toprule
 & de-pearson-6k & es-pearson-6k & jina-zh & multilingual-e5-base \\
\midrule
mean & 0.688 & 0.690 & 0.677 & \bfseries 0.730 \\
AmazonCounterfactualClassification (en) & 0.740 & 0.743 & 0.722 & \bfseries 0.790 \\
AmazonPolarityClassification (en) & 0.802 & 0.783 & 0.720 & \bfseries 0.906 \\
AmazonReviewsClassification (en) & 0.395 & 0.383 & 0.354 & \bfseries 0.445 \\
Banking77Classification (en) & 0.839 & \bfseries 0.853 & 0.842 & 0.827 \\
EmotionClassification (en) & 0.452 & 0.466 & \bfseries 0.473 & 0.452 \\
ImdbClassification (en) & 0.699 & 0.675 & 0.696 & \bfseries 0.855 \\
MTOPDomainClassification (en) & 0.903 & 0.904 & 0.894 & \bfseries 0.931 \\
MTOPIntentClassification (en) & 0.686 & 0.720 & 0.695 & \bfseries 0.753 \\
MassiveIntentClassification (en) & 0.696 & 0.708 & 0.696 & \bfseries 0.721 \\
MassiveScenarioClassification (en) & 0.741 & 0.738 & 0.740 & \bfseries 0.771 \\
ToxicConversationsClassification (en) & 0.695 & \bfseries 0.700 & 0.695 & 0.698 \\
TweetSentimentExtractionClassification (en) & \bfseries 0.613 & 0.611 & 0.594 & \bfseries 0.613 \\
\bottomrule
\end{tabular}

==> tables/english/clustering.tex <==
\begin{tabular}{lcccc}
\toprule
 & de-pearson-6k & es-pearson-6k & jina-zh & multilingual-e5-base \\
\midrule
mean & 0.403 & \bfseries 0.405 & 0.368 & 0.400 \\
ArxivClusteringP2P (en) & \bfseries 0.419 & 0.415 & 0.405 & 0.403 \\
ArxivClusteringS2S (en) & 0.325 & 0.322 & 0.315 & \bfseries 0.354 \\
BigPatentClustering (en) & 0.230 & 0.204 & 0.187 & \bfseries 0.240 \\
BiorxivClusteringP2P (en) & 0.344 & \bfseries 0.352 & 0.296 & 0.350 \\
BiorxivClusteringS2S (en) & 0.290 & 0.289 & 0.278 & \bfseries 0.295 \\
MedrxivClusteringP2P (en) & 0.316 & \bfseries 0.322 & 0.272 & 0.289 \\
MedrxivClusteringS2S (en) & \bfseries 0.294 & 0.288 & 0.263 & 0.284 \\
RedditClustering (en) & 0.479 & \bfseries 0.483 & 0.426 & 0.424 \\
RedditClusteringP2P (en) & 0.549 & \bfseries 0.560 & 0.530 & 0.552 \\
StackExchangeClustering (en) & \bfseries 0.555 & 0.554 & 0.532 & 0.553 \\
StackExchangeClusteringP2P (en) & 0.328 & \bfseries 0.336 & 0.325 & 0.305 \\
TwentyNewsgroupsClustering (en) & \bfseries 0.405 & 0.402 & 0.351 & 0.360 \\
WikiCitiesClustering (en) & 0.703 & 0.733 & 0.604 & \bfseries 0.796 \\
\bottomrule
\end{tabular}


==> tables/english/pair-classification.tex <==
\begin{tabular}{lcccc}
\toprule
 & de-pearson-6k & es-pearson-6k & jina-zh & multilingual-e5-base \\
\midrule
mean & 0.835 & \bfseries 0.846 & 0.815 & 0.836 \\
SprintDuplicateQuestions (en) & 0.940 & \bfseries 0.956 & 0.932 & 0.930 \\
TwitterSemEval2015 (en) & 0.705 & 0.716 & 0.665 & \bfseries 0.722 \\
TwitterURLCorpus (en) & 0.860 & \bfseries 0.864 & 0.849 & 0.855 \\
\bottomrule
\end{tabular}


==> tables/english/reranking.tex <==
\begin{tabular}{lcccc}
\toprule
 & de-pearson-6k & es-pearson-6k & jina-zh & multilingual-e5-base \\
\midrule
mean & 0.549 & \bfseries 0.553 & 0.550 & 0.548 \\
AskUbuntuDupQuestions (en) & \bfseries 0.612 & \bfseries 0.612 & 0.610 & 0.582 \\
MindSmallReranking (en) & 0.303 & 0.306 & \bfseries 0.311 & 0.310 \\
SciDocsRR (en) & 0.786 & 0.793 & 0.786 & \bfseries 0.807 \\
StackOverflowDupQuestions (en) & 0.496 & \bfseries 0.502 & 0.492 & 0.494 \\
\bottomrule
\end{tabular}


==> tables/english/retrieval.tex <==
\begin{tabular}{lcccc}
\toprule
 & de-pearson-6k & es-pearson-6k & jina-zh & multilingual-e5-base \\
\midrule
mean & 0.441 & 0.464 & 0.460 & \bfseries 0.489 \\
ArguAna (en) & 0.495 & \bfseries 0.501 & 0.395 & 0.442 \\
CQADupstackRetrieval (en) & 0.368 & \bfseries 0.388 & 0.365 & 0.385 \\
ClimateFEVER (en) & 0.222 & \bfseries 0.271 & 0.233 & 0.239 \\
DBPedia (en) & 0.320 & 0.326 & 0.302 & \bfseries 0.404 \\
FEVER (en) & 0.712 & 0.784 & 0.786 & \bfseries 0.794 \\
FiQA2018 (en) & 0.339 & 0.370 & 0.349 & \bfseries 0.382 \\
HotpotQA (en) & 0.548 & 0.595 & 0.603 & \bfseries 0.686 \\
MSMARCO (en) & 0.345 & 0.355 & 0.407 & \bfseries 0.423 \\
NFCorpus (en) & 0.280 & 0.303 & 0.308 & \bfseries 0.325 \\
NQ (en) & 0.481 & 0.507 & 0.594 & \bfseries 0.600 \\
QuoraRetrieval (en) & 0.877 & 0.881 & \bfseries 0.885 & 0.876 \\
SCIDOCS (en) & 0.167 & 0.174 & \bfseries 0.179 & 0.172 \\
SciFact (en) & 0.609 & 0.627 & 0.612 & \bfseries 0.693 \\
TRECCOVID (en) & 0.648 & 0.674 & 0.638 & \bfseries 0.698 \\
Touche2020 (en) & 0.205 & 0.198 & \bfseries 0.242 & 0.214 \\
\bottomrule
\end{tabular}


==> tables/english/sts.tex <==
\begin{tabular}{lcccc}
\toprule
 & de-pearson-6k & es-pearson-6k & jina-zh & multilingual-e5-base \\
\midrule
mean & 0.820 & \bfseries 0.835 & 0.826 & 0.803 \\
BIOSSES (en) & 0.780 & 0.830 & 0.805 & \bfseries 0.851 \\
SICK-R (en) & 0.811 & 0.830 & \bfseries 0.862 & 0.785 \\
STS12 (en) & 0.801 & 0.816 & \bfseries 0.874 & 0.767 \\
STS13 (en) & 0.851 & \bfseries 0.868 & 0.818 & 0.780 \\
STS14 (en) & 0.811 & \bfseries 0.836 & 0.786 & 0.766 \\
STS15 (en) & 0.878 & \bfseries 0.887 & 0.861 & 0.882 \\
STS16 (en) & 0.836 & \bfseries 0.860 & 0.841 & 0.843 \\
STS17 (en) & \bfseries 0.893 & 0.886 & 0.886 & 0.878 \\
STS22 (en) & \bfseries 0.682 & 0.656 & 0.672 & 0.618 \\
STSBenchmark (en) & 0.862 & \bfseries 0.878 & 0.858 & 0.856 \\
\bottomrule
\end{tabular}

==> tables/english/summarization.tex <==
\begin{tabular}{lcccc}
\toprule
 & de-pearson-6k & es-pearson-6k & jina-zh & multilingual-e5-base \\
\midrule
mean & \bfseries 0.318 & 0.299 & 0.313 & 0.301 \\
SummEval (en) & \bfseries 0.318 & 0.299 & 0.313 & 0.301 \\
\bottomrule
\end{tabular}


==> tables/german/classification.tex <==
\begin{tabular}{lcc}
\toprule
 & de-pearson-6k-lang-de & multilingual-e5-base-de \\
\midrule
mean & 0.665 & \bfseries 0.687 \\
AmazonCounterfactualClassification (de) & 0.692 & \bfseries 0.717 \\
AmazonReviewsClassification (de) & 0.385 & \bfseries 0.418 \\
MTOPDomainClassification (de) & 0.892 & \bfseries 0.896 \\
MTOPIntentClassification (de) & 0.653 & \bfseries 0.712 \\
MassiveIntentClassification (de) & 0.650 & \bfseries 0.661 \\
MassiveScenarioClassification (de) & 0.718 & \bfseries 0.720 \\
\bottomrule
\end{tabular}

==> tables/german/clustering.tex <==
\begin{tabular}{lcc}
\toprule
 & de-pearson-6k-lang-de & multilingual-e5-base-de \\
\midrule
mean & 0.299 & \bfseries 0.328 \\
BlurbsClusteringP2P (de) & 0.349 & \bfseries 0.394 \\
BlurbsClusteringS2S (de) & \bfseries 0.167 & 0.157 \\
TenKGnadClusteringP2P (de) & 0.431 & \bfseries 0.439 \\
TenKGnadClusteringS2S (de) & 0.250 & \bfseries 0.320 \\
\bottomrule
\end{tabular}


==> tables/german/pair-classification.tex <==
\begin{tabular}{lcc}
\toprule
 & de-pearson-6k-lang-de & multilingual-e5-base-de \\
\midrule
mean & \bfseries 0.583 & 0.541 \\
PawsX (de) & \bfseries 0.583 & 0.541 \\
\bottomrule
\end{tabular}

==> tables/german/reranking.tex <==
\begin{tabular}{lcc}
\toprule
 & de-pearson-6k-lang-de & multilingual-e5-base-de \\
\midrule
mean & 0.639 & \bfseries 0.648 \\
MIRACL (de) & 0.639 & \bfseries 0.648 \\
\bottomrule
\end{tabular}

==> tables/german/retrieval.tex <==
\begin{tabular}{lcc}
\toprule
 & de-pearson-6k-lang-de & multilingual-e5-base-de \\
\midrule
mean & \bfseries 0.387 & 0.342 \\
GerDaLIR (de) & \bfseries 0.172 & 0.069 \\
GermanDPR (de) & \bfseries 0.795 & \bfseries 0.795 \\
XMarket (de) & \bfseries 0.195 & 0.163 \\
\bottomrule
\end{tabular}

==> tables/german/sts.tex <==
\begin{tabular}{lcc}
\toprule
 & de-pearson-6k-lang-de & multilingual-e5-base-de \\
\midrule
mean & \bfseries 0.714 & 0.674 \\
GermanSTSBenchmark (de) & \bfseries 0.845 & 0.789 \\
STS22 (de) & \bfseries 0.583 & 0.560 \\
\bottomrule
\end{tabular}

==> tables/spanish/classification.tex <==
\begin{tabular}{lcc}
\toprule
 & es-pearson-6k & multilingual-e5-base \\
\midrule
mean & 0.671 & \bfseries 0.685 \\
AmazonReviewsClassification (es) & 0.387 & \bfseries 0.405 \\
MTOPDomainClassification (es) & 0.899 & \bfseries 0.906 \\
MTOPIntentClassification (es) & 0.688 & \bfseries 0.713 \\
MassiveIntentClassification (es) & 0.669 & \bfseries 0.684 \\
MassiveScenarioClassification (es) & 0.712 & \bfseries 0.715 \\
\bottomrule
\end{tabular}

==> tables/spanish/clustering.tex <==
\begin{tabular}{lcc}
\toprule
 & es-pearson-6k & multilingual-e5-base \\
\midrule
mean & \bfseries 0.440 & 0.413 \\
FloresClusteringS2S (es) & \bfseries 0.398 & 0.367 \\
SpanishNewsClusteringP2P (es) & \bfseries 0.483 & 0.458 \\
\bottomrule
\end{tabular}

==> tables/spanish/pair-classification.tex <==
\begin{tabular}{lcc}
\toprule
 & es-pearson-6k & multilingual-e5-base \\
\midrule
pair-classification average & \bfseries 0.590 & 0.551 \\
PawsX (es) & \bfseries 0.590 & 0.551 \\
\bottomrule
\end{tabular}

==> tables/spanish/reranking.tex <==
\begin{tabular}{lcc}
\toprule
 & es-pearson-6k & multilingual-e5-base \\
\midrule
mean & \bfseries 0.739 & 0.736 \\
MIRACL (es) & \bfseries 0.739 & 0.736 \\
\bottomrule
\end{tabular}

==> tables/spanish/retrieval.tex <==
\begin{tabular}{lcc}
\toprule
 & es-pearson-6k & multilingual-e5-base \\
\midrule
mean & \bfseries 0.511 & 0.478 \\
MIRACLRetrieval (es) & 0.809 & \bfseries 0.820 \\
MintakaESRetrieval (es) & 0.283 & \bfseries 0.299 \\
SpanishPassageRetrievalS2P (es) & \bfseries 0.421 & 0.394 \\
SpanishPassageRetrievalS2S (es) & \bfseries 0.704 & 0.654 \\
XMarketES (es) & \bfseries 0.197 & 0.119 \\
XPQAESRetrieval (es) & \bfseries 0.654 & 0.583 \\
\bottomrule
\end{tabular}

==> tables/spanish/sts.tex <==
\begin{tabular}{lcc}
\toprule
 & es-pearson-6k & multilingual-e5-base \\
\midrule
mean & \bfseries 0.788 & 0.783 \\
STS17 (es) & \bfseries 0.882 & 0.867 \\
STS22 (es) & \bfseries 0.680 & 0.666 \\
STSES (es) & 0.802 & \bfseries 0.816 \\
\bottomrule
\end{tabular}
